Quantum limits of superconducting-photonic links and their extension to mm-waves

Photonic addressing of superconducting circuits has been proposed to overcome wiring complexity and heat load challenges, but superconducting-photonic links suffer from an efficiency-noise trade-off that limits scalability. This trade-off arises because increasing power conversion efficiency requires reducing optical power, which makes the converted signal susceptible to shot noise. We analyze this trade-off and find the infidelity of qubit gates driven by photonic signals scales inversely with the number of photons used, and therefore the power efficiency of the converter. While methods like nonlinear detection or squeezed light could mitigate this effect, we consider generating higher frequency electrical signals, such as millimeter-waves (100 GHz), using laser light. At these higher frequencies, circuits have higher operating temperatures and cooling power budgets. We demonstrate an optically-driven cryogenic millimeter-wave source with a power efficiency of $10^{-4}$ that can generate ${1}~\mathrm{\mu W}$ of RF power at 80 GHz with 1500 thermal photons of added noise at 4 K. Using this source, we perform frequency-domain spectroscopy of superconducting NbTiN resonators at 80-90 GHz. Our results show a promising approach to alleviate the efficiency-noise constraints on optically-driven superconducting circuits while leveraging the benefits of photonic signal delivery. Further optimization of power efficiency and noise at high frequencies could make photonic control of superconducting qubits viable at temperatures exceeding 1 kelvin.

==> unused.tex <==
%%% UNUSED / TRASH

%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines

% \usepackage[showframe,%Uncomment any one of the following lines to test 
% % scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
% %text={7in,10in},centering,
% %margin=1.5in,
% %total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
% %height=10in,a5paper,hmargin={3cm,0.8in},
% ]{geometry}

%\title{Superconducting-Photonic Links: Limitations and Extension to mm-Waves}
% \title{Addressing the Limitations of Superconducting-Photonic Links using Millimeter-Waves}
%\title{Addressing the Limitations of Optically Controlled Superconducting Qubits with Millimeter-Waves}
% \title{Optically Driven Cryogenic Microwave Devices: Strategies, Limitations, and Application in mm-Wave Signals}

%Photonic addressing of superconducting qubit systems has been proposed as an approach to overcome the tyranny of wires in emerging cryogenic microwave quantum technologies, and the associated wiring and heating challenges.  We reveal an efficiency-noise trade-off in superconducting-photonic links, which affects the scalability of approaches that use photodiodes to generate microwave signals. This trade-off is fundamentally due to the uncertainty of photon number in a coherent optical field. We find that single-qubit gate error probability scales as $1/N_\text{opt, tot}$, where $N_\text{opt, tot}$ is the total number of optical photons used in the gate and that this trade-off significantly limits the scalability of photonic-superconducting links. While more complex methods, such as nonlinear detection, intensity-squeezed light, or coherent conversion may circumvent this quantum noise limit, we consider an alternate question: does increasing the RF frequency of superconducting-photonic links help? Higher frequency superconducting systems enable higher temperature operation and greater heat budgets, favorably modifying the scalability calculus. Thus, we build an optically driven cryogenic millimeter-wave source and demonstrate frequency-domain spectroscopy of thin-film NbTiN superconducting resonators in the $80$ -- $90$ GHz range. Our source can generate roughly \SI{1}{\micro\watt} of RF power at 80 GHz in a $\SI{4}{\K}$ environment, using \SI{10}{\milli\watt} of optical power; corresponding to a power efficiency of $10^{-4}$ and with added noise equivalent to $1500$ thermal photons. 

%The generated RF power is $P_\text{RF} = \frac{1}{2}Z_0\mathcal{R}^2P_0^2|\mathcal{H}(\Omega)|^2$, where $\mathcal{H}(\Omega)$ is the transfer function of the photodiode.

% In the sections below we provide details on an experimental implementation of optically-driven signals to probe a superconducting mm-wave resonator.

%To meet the demands of fault-tolerant quantum computing in superconducting systems in the face of a 10 microwatt power budget is a monumental challenge. Given the additional efficiency-noise trade off, control of qubits using microwave photonics is fundamentally limited without advanced solutions such as nonlinear detection, intensity-squeezed light, or direct quantum frequency conversion. Therefore, exploring solutions that increase the power budget, such as higher temperature and RF frequency operation are attractive. While the efficiency-noise trade off still exists at higher RF frequencies, it is less pronounced due to the increased cooling power. So, in this work we focus our effort in building and characterizing an optically-driven millimeter-wave source inside of a dilution refrigerator. In the following sections, we provide details on the cryogenic photogeneration of mm-wave signals and using these signals to probe a superconducting mm-wave resonator.

%We couple mm-wave superconducting circuits to the fundamental TE mode of a WR10 rectangular waveguide~\cite{stokowski2019towards, multani2020development, anferov2020millimeter}. To probe these circuits with a high-speed photodiode (HSPD), we use an adapter. The adapter transitions the RF generated by the HSPD's output into the rectangular waveguide, as shown in~\hyperef{Figure}{fig:princop}. Additionally,~\hyperef{Figure}{fig:princop} shows a schematic of the power spectrum at the input of the HSPD and the output of the rectangular waveguide. The output spectrum has a natural bandwidth set by a lower cutoff frequency of the rectangular waveguide and an upper cutoff frequency set by the bandwidth of the HSPD.

%Due to the high bandwidth and low passive thermal load of optical fibers, many RF signals can be generated within a cryogenic environment~\cite{lecocq2021control}.~\hyperef{Figure}{fig:princop} shows two situations where multiple RF signals with can be generated and distributed within a cryostat. The first situation is to use electro-optic modulators (EOMs) to modulate a carrier laser so that the sidebands beat on the photodiode mounted in a cryogenic environment. The second situation is to generate the RF signals using an optical frequency comb~\cite{capmany2007microwave,feng2024integrated,kudelin2024photonic,sun2024integrated,stokowski2024integrated}. In both cases, any phase noise in the optical fields beats on the photodiode and cancels out.

% If we attribute all of the insertion loss at $\SI{3.09}{\K}$ to the HSPD magnitude response at 80 GHz, then the HSPD bandwidth is no less than $\SI{70}{\GHz}$, given the independent room temperature bandwidth measurement of $75$ GHz shown in~\hyperef{Figure}{fig:HSPD} (c).

 %(b) General cryogenic operation of the optically-driven source. The HSPD and adapter can be mounted in a low-temperature and pressure environment. The optical input can have many coherent tones from a set of electro-optic modulators or optical frequency combs.}


%% Room temperature: 10log10(|L(w)|^2) = -19.66 dB +/- 0.44 dB
%% Base temperature: 10log10(|L(w)|^2) = -7.5 dB +/- 0.44 dB

% room T power fit: 0.5*ax^2  => a = 0.0863 +/- 9.1773e-04,
% base T power fit: 0.5*ax^2  => a = 0.0219 +/- 2.9378e-04

% S RT = 2150 mV/mW
% S BT = 4649 mV/mW


% Additionally, we observed the expected quadratic dependence in the generated power and observed above 1 microwatts of 80 GHz power in a 4 K environment. The error bars in the cryogenic data originate from uncertainty in the cryogenic sensitivity of the mm-wave detector (see Appendix B).

%We measured the detection efficiency by measuring the IF power generated for a given mm-wave power, i.e., $P_\text{500 MHz} = G_\text{det} P_\text{80 GHz}$. We find $G_\text{det} = 0.51$. This detection efficiency is also incorporated to the theoretical shot-noise shown in~\hyperef{Figure}{fig:pwrnoise} (b). 

%The measured noise is approximately ten times higher than the output-referred shot-noise limit at the lowest optical power and scales quadratically with optical power. We fit the data with a quadratic fit (blue dashed lined), $f(x) = ax^2+b$, where $a = 1.63 \cdot 10^{-15}\text{ }\SI{}{\watt\per\Hz\per\watt\squared}$ and $b = 2.45\cdot 10^{-21} \text{ }\SI{}{\watt\per\Hz} $. Note, we cannot distinguish this quadratic scaling (coming from excess noise) from the increased relative intensity noise of the laser signal post-EDFA amplification and operating above the photodiode's bandwidth~\cite{putra2017edfanoise,lecocq2021control}. 

% Additionally, it is important to note that we found the harmonic mixer to add the most amount of noise to our detection chain. The mixer's conversion gain is at most $-56.4 \text{ dB}$ and its noise figure to be at most $41 \text{ dB}$ at cryogenic temperatures. 

% The associated readout fidelity is,
% \begin{align}
%     F_\text{r} &= 1 - \frac{1}{2}P(0|1) - \frac{1}{2}P(1|0)\\
%     &=  1 - \left(\frac{\pi}{2}\right)^2 \frac{1}{N_\text{tot,opt}},
% \end{align}
% where $P(0|1)$ is the probability of measuring $\ket{0}$ given that we prepared $\ket{1}$ \textit{i.e.} the error probability. Similar for $P(1|0)$.

% \begin{figure}[ht!]
% \centering
% \includegraphics[width=\linewidth]{Figures/IF_pwr_vs_RF_pwr_20230918.pdf}
% \caption{\label{fig:gaincalibration}This figure shows the gain calibration curve. Same experimental setup as shown in Figure 3c.}
% \end{figure}


%Utilizing millimeter-waves (mm-waves) in quantum hardware has recently been accumulating interest. These frequencies (30 GHz--300 GHz) present exciting possibilities for quantum information science and technology, as they could enable enhanced light-matter interactions in various physical systems. Quantum optomechanics~\cite{hauer2021quantum}, millimeter-wave superconducting qubits~\cite{anferov2020millimeter, faramarzi2021initial}, Rydberg atoms, and quantum frequency transduction~\cite{pechal2017millimeter,mckenna2020cryogenic,kumar2023quantum} are all currently being explored as areas where using mm-waves could provide advantages. However, practical challenges exist in harnessing mm-waves for applications requiring superconducting circuits. Sending mm-waves into cryostats, essential for maintaining superconducting circuits at low temperatures, is challenging~\cite{krinner2019engineering}. Traditional rectangular waveguides, while effective, introduce high passive heat loads and are bulky~\cite{magnard2020microwave}. On the other hand, coaxial waveguides, although compact, become increasingly lossy and costly as the frequency increases~\cite{kurpiers2017characterizing}. 

%We characterize the power and noise properties of the detection chain. Lastly, we perform frequency domain spectroscopy of superconducting mm-wave antenna resonators using the source~\cite{stokowski2019towards, multani2020development, anferov2020millimeter}.

%Such demonstrations show that optically-driven techniques meet the experimental demands of quantum information processing while leveraging optical fibers' low loss and high bandwidth properties. 

%Shot-noise impacts a quantum computing system by degrading qubit performance and limiting the number of gates one can apply. It is well known that a qubit's dephasing rate, $\Gamma_\phi$, increases due to the effective temperature increase of the surrounding bath~\cite{clerk2007using, reagor2016quantum,lecocq2021control}. However, considerations regarding how shot-noise introduces uncertainty in qubit control have yet to be discussed.  

%In this work, we build an optically-driven mm-wave source and use it to measure superconducting mm-wave circuits. The source consists of one diode laser in the optical C-band (1550 nm), a high-bandwidth electro-optic modulator, and a high-speed photodiode. The photodiode is mounted on the 4 K stage of a cryostat, where the mm-waves are generated~\cite{Zhang1997cryogenic, huggard2007photonic, bardalen2018evaluation}. We characterize the power and noise properties of the detection chain. Lastly, we perform frequency domain spectroscopy of superconducting mm-wave antenna resonators using the source~\cite{stokowski2019towards, multani2020development, anferov2020millimeter}.

% \section{Power and noise modeling}
% \label{appendix:pwrnoisemodel}
% \subsection{Two-tones}
% In this section, we show a semi-classical model of the system; what we are after is the power spectral density of the photocurrent given two optical fields. In the simplest case, we have two coherent laser fields $\alpha_1(t)= \frac{A_1}{2}\left(e^{i\omega_1 t}+ e^{-i\omega t}\right)$, $\alpha_2(t)=\frac{A_2}{2}\left(e^{i\omega_2 t}+ e^{-i\omega_2 t}\right)$, and a noise process $\alpha_n(t)$. The noise term is used to model the vacuum fluctuations in the optical field; the noise is Gaussian and has the following properties: $\langle \alpha_n(t) \rangle = \langle\alpha_n(t)\alpha_n(t')\rangle= 0$ and $\langle\alpha_n(t)\alpha_n(t')^\ast\rangle = N \delta(t-t')$,  where $N$ is a normalization factor. In total we have, $\alpha(t) = \alpha_1(t) + \alpha_2(t) + \alpha_n(t)$. Note the field amplitudes can be renormalized so that $A_1$ and $A_2$ have units of $\sqrt{\text{watts}}$, therefore, the optical power can  be written as $P(t)=\alpha^\ast(t)\alpha(t)$. In our case, the power is (ignoring the DC term and fast oscillating terms),
% \begin{align}
%     P(t) &= A_1A_2\cos\left(\omega_{-}t\right) \\
%     &+ (\alpha_n(t) + \alpha_n^\ast(t))\left(A_1\cos(\omega_1 t)+A_2\cos(\omega_2 t)\right) \nonumber,
% \end{align}
% where $\omega_{-} = \omega_1-\omega_2$ is the beat frequency. When this impinges onto a photodiode, the photocurrent generated is $I(t) = \mathcal{G} P(t)$, where $\mathcal{G}$ is the photodiode gain. In general, the two-sided power spectral density of a measurable, $X(t)$, is defined as 
% \begin{align}
%     S_{XX}(\Omega) &= \int_{-\infty}^{\infty} e^{i\Omega \tau} X^\ast(t) X(t-\tau) d\tau \\
%     &= \int_{-\infty}^{\infty} X^\ast(\Omega)X(\Omega')d\Omega',
% \end{align}
% where $X(\Omega)$ is the Fourier transform of $X(t)$.  Note, $S_{II}(\Omega) = \mathcal{G}^2 S_{PP}(\Omega)$. First, we compute the Fourier transform of $P(t)$, 
% \begin{align}
%     P(\Omega) &= \frac{A_1A_2}{2}\Big(\delta(\Omega-\omega_-) + \delta(\Omega+\omega_{-})\Big) \nonumber \\
%     &+ \frac{A_1}{2}\Big(\alpha_n(\Omega-\omega_1) + \alpha_n(\Omega+\omega_1) + \text{c.c}\Big) \nonumber \\
%     &+ \frac{A_2}{2}\Big(\alpha_n(\Omega-\omega_2) + \alpha_n(\Omega+\omega_2) + \text{c.c}\Big),
% \end{align}
% where $\alpha_n(\Omega)$ is the Fourier transform of $\alpha_n(t)$.  So, in total, we get the two-sided power spectral density of the optical power to be,
% \begin{align}
%     S_{PP}(\Omega) &= \frac{A_1^2A_2^2}{2}\Big(\delta(\Omega-\omega_-) + \delta(\Omega+\omega_{-})\Big) \nonumber \\
%     &+ \frac{NA_1^2}{2} \nonumber \\
%     &+ \frac{NA_2^2}{2}.
% \end{align}
% Finally, we can write down the power spectral density of the photocurrent.
% \begin{align}
%     S_{II}(\Omega) &= \underbrace{\mathcal{G}^2\frac{A_1^2A_2^2}{2}\delta(\Omega-\omega_{-})}_{\text{RF}} + \underbrace{\mathcal{G}^2\frac{NA_1^2}{2} + \mathcal{G}^2\frac{NA_2^2}{2}}_\text{shot noise}.
% \end{align}
%  Since the spectrum analyzer only measures positive frequencies, $\Omega$, we neglect the $\delta(\Omega+\omega_{-})$ term. Here, we find that there is an RF frequency at $\omega_{-} = \omega_1 - \omega_2$. If the optical powers of the two tones are equal, we find that the RF power scales quadratically with the optical power. In this case, each optical field contributes its own portion to the shot noise.

% \subsection{Many-tones}
% In the previous section, we considered two coherent optical fields impinging onto the photodiode. Generally speaking, we can have many coherent fields. We can generate these  fields by modulating the light to generate sidebands or by utilizing an optical frequency comb. In either case, we have the total optical field of $M$ tones, $ \alpha(t) = \sum_{n=0}^{M}A_n \cos(\omega_n t)$. The total optical power is,
% \begin{align}
%   P(t) &= \Big(\sum_{n=0}^{M} A_n^\ast\cos(\omega_n t)\Big) \Big(\sum_{n=0}^{M} A_n\cos(\omega_n t)\Big),\nonumber \\
%   &= \sum_{n=0}^{M}\sum_{k=0}^{n} A_n^\ast A_{n-k}\cos(\omega_n t)\cos(\omega_{n-k}t), \nonumber \\
%   & = \frac{1}{2}\sum_{n=0}^{M}\sum_{k=0}^{n} A_n^\ast A_{n-k}\Big(\cos([\omega_n-\omega_{n-k}] t) \nonumber \\ 
%   &+\cos([\omega_n+\omega_{n-k}]t)\Big).
% \end{align}
% From this expression, we deduce that the RF spectrum will have all beat frequencies $\omega_n-\omega_{n-k}$  within the bandwidth of the photodiode.

% The shot-noise term in this case follows directly from above; every additional optical field linearly adds its own contribution,
% \begin{align}
%     S_{II}^{\text{shot}}(\Omega) &= \mathcal{R}^2\sum_{n=0}^{M} \frac{N |A_n|^2}{2}.
% \end{align}


\label{sec:noise}
% \subsection{Derivation of Photocurrent Shot Noise}
% \label{subsec:photocurrentnoise}
% Consider measurements of a photocurrent generated by light with frequency $\omega$, on a photodiode with responsivity $\mathcal{R}=\frac{e_0}{\hbar\omega}$, where $e_0$ is the electron charge. For an ideal photoelectric detector, one electron is produced for each photon in a measurement time interval $T$. This interval $T$ is set by the detection electronics. We can define an observable, $\hat{i}_T = e_0 \frac{\hat{N}}{T}$, where $\hat{N}$ is the number operator, $\hat{N}=\hat{a}^\dagger\hat{a}$. Taking the expected value of the observable, given that the input state is a coherent state, we get,
% \begin{equation}
% \langle \hat{i}_T \rangle = e_0 \frac{\langle\alpha|\hat{N}|\alpha\rangle}{T} = \frac{e_0}{T} |\alpha|^2 = e_0 n_0/T = e_0 \frac{P_0}{\hbar\omega} = i_0
% \end{equation}
% where $\dot{n}_0=n_0/T$ (${P}_0$) is the average photon flux (laser power) and $e_0$ is the electron charge. Here we note the responsivity is $\mathcal{R}=e_0/(\hbar\omega)$. The angle brackets indicate two averages: a time average over the interval $T$ and an ensemble average. Recall that the variance is defined as,
% \begin{equation}
%     \text{Var}\left( \hat{i}_T \right) = \langle \hat{i}^2_T \rangle - \langle \hat{i}_T \rangle ^2.
% \end{equation}
% The second moment of the current operator is $\langle \alpha | \hat{i}^2_T | \alpha \rangle = (\frac{e_0}{T})^2\left(|\alpha|^4 + |\alpha|^2\right)$, where $|\alpha|^2 = n_0 = \dot{n}_0 T $.
% Therefore, 
% \begin{equation}
%     \text{Var}\left(\hat{i}_T\right) = \left(\frac{e_0}{T}\right)^2 |\alpha|^2 = e_0\frac{\mathcal{R}P_0}{T} = \frac{e_0i_0}{T}
% \end{equation}
% The measurement interval $T$ (i.e. integration time) is set by the bandwidth of the detection electronics $\Delta \omega = \frac{2\pi}{T}$.
% Therefore the variance of our current operator is,
% \begin{equation}
%     \text{Var}\left(\hat{i}_T\right) = e_0 {i}_0\Delta \omega/(2\pi).
% \end{equation}
% For each measurement in the lab, we expect the measured current to be,
% \begin{equation}
%     i = {i}_0 + i_{n}
% \end{equation}
% where $i_{n}$ is a sample from Gaussian distribution with $\mu = 0$ and $\sigma^2 = \text{Var}\left(\hat{i}_T\right)$. For such noise processes, the auto-correlation function is given by $R_{ii}(t) = \sigma^2 \delta(t)$.
% The Fourier transform of this auto-correlation function gives the double-sided power spectral density (Wiener-Khinchin),
% \begin{equation}
% {S}_{ii}^{\text{shot-noise}} = \int_{-\infty}^{\infty} d\tau e^{-i\omega \tau} R_{ii}(\tau) d\tau = \sigma^2
% \end{equation}
% Therefore, the double-sided power spectral density is,
% \begin{equation}
%     {S}_{ii}^{\text{shot-noise}}=\text{Var}(\hat{i}_T) = e_0 {i}_0 = e_0\mathcal{R}P_0 \Delta f
% \end{equation}
% which agrees with Schottky's result~\cite{schottky2018spontaneous,lecocq2021control}. In the main text we let $\Delta f = \SI{1}{\Hz}$. For a non-ideal photodiode, the same power spectral formula holds. However, measured photocurrent suffers for the same input power,
% \begin{equation}
%     \mathcal{R} \to \eta_\text{q}\mathcal{R}
% \end{equation}
% where $\eta_{\text{q}} \le 1$ is the quantum efficiency of the detector. This is saying that the probability that an electron is generated decreases for the same input photon flux. The above analysis holds for coherent states/constant intensity fields. In total, we have
% \begin{equation}
%     {S}_{ii}^{\text{shot-noise}} = e_0\eta_\text{q}\mathcal{R}P_0,
% \end{equation}
% which is the expression we use in Section~\ref{sec:effectivetemp}.

% \subsection{Derivation of Thermal Noise of a Passive Electronic Device}
% \label{subsec:jnnoise}
% Here, we sketch a derivation of the noise of a thermal source (Johnson-Nyquist) we used in Section~\ref{sec:effectivetemp}, using the fluctuation-dissipation theorem. Suppose we have a circuit element in thermal equilibrium with a bath held at temperature $T$. Suppose we can inject charges $q(t)$ into the element. This leads to an interaction energy, $-q(t)\hat{V}$ where $\hat{V}$ is the voltage operator. Linear response theory tells us that the expectation value of the voltage operator is given by,
% \begin{equation}
%     \langle \hat{V} \rangle = \int_{-\infty}^\infty q(t-\tau) \chi_{VV}(\tau) \mathrm d \tau,
% \end{equation}
% where $\chi_{VV}(t)$ is the linear response function of the circuit element. In fourier domain, we have
% \begin{equation}
%     \langle \hat{V} \rangle(\omega) = V(\omega) =  q(\omega) \chi_{VV}(\omega).
% \end{equation}
% The current in the fourier domain is $I(\omega) = i\omega q(\omega)$. Therefore, we get
% \begin{equation}
%     V(\omega) = \chi_{VV}(\omega)/(i\omega) \cdot I(\omega) \implies \chi_{VV} = i \omega Z(\omega).
% \end{equation}
% From the fluctuation-dissipation theorem, we can write the double-sided power spectral density as,
% \begin{equation}
%     S_{VV} (\omega) = \hbar \coth\left(\frac{\beta\hbar\omega}{2}\right)\text{Im}[\chi_{VV}(\omega)],
% \end{equation}
% where $\beta = 1/(kT)$, $k$ is Boltzmann's constant. In our case, the element is a photodiode and is coupled to an electromagnetic environment with characteristic impedance $Z_0$, i.e. $Z(\omega) = Z_0$. Combining the previous two equations results in,
% \begin{equation}
%     S_{VV}(\omega) = \hbar\omega\coth\left(\frac{\beta\hbar\omega}{2}\right)Z_0.
% \end{equation}
%  Finally, using the relation $S_{II} = S_{VV}/Z_0^2$, we arrive at
%  \begin{equation}
%      S_{II}^{\text{thermal,q}}(\omega)  = \hbar\omega\coth\left(\frac{\hbar\omega}{2kT}\right)\frac{1}{Z_0}.
%  \end{equation}
%  Note, in the thermodynamic limit $\hbar\omega \ll k T$ we recover the Johnson-Nyquist result of $2kT/Z_0$ (note there is a factor of two because this is the double-sided power spectral density).

% \section{IF Phase Noise Measurements}
% \label{appendix:mixerphasenoise}


% \begin{figure}[ht!]
% \centering
% \includegraphics[width=\linewidth]{Figures/ssb_phase_noise_20240109.pdf}
% \caption{\label{fig:phasenoise}This figure shows the SSB phase noise of the 500 MHz signal, mixed down from 80 GHz using the harmonic mixer. Same experimental setup as shown in F.}
% \end{figure}

%The broadband noise power of the source is approximately ten times higher than expected from the shot-noise limit, which we cannot distinguish between an increase in relative-intensity noise after the EDFA (due to amplified spontaneous emission) and operating above the HSPD's bandwidth. 

% Improvements can be made on several different aspects of the source. To increase the generated RF power and increase the frequency range of operation, it is important to maintain high responsivity at cryogenic temperatures, drive the EOM with higher power, use a higher bandwidth EOM, and use a higher bandwidth HSPD. These improvements will also help with the excess noise problems as the EDFA can be removed, reducing the relative intensity noise~\cite{putra2017edfanoise}. Lastly, we found that the detection chain is greatly impacted by the gain ($-55$ dB) and noise figure ($35$ dB) of the harmonic mixer, used to down-convert the mm-waves to microwaves (see~\hyperef{Appendix}{appendix:mixernoise}). The mixer's cryogenic performance underscores the need for high internal efficiency superconducting millimeter-wave mixers, which can be useful in both classical and quantum applications.

%The observed excess noise could pose problems for quantum control of a mm-wave qubit, as increased noise reduces the ground state population~\cite{clerk2007using, reagor2016quantum}. To mitigate this excess noise, several strategies could be effective: increasing the HSPD bandwidth, improving the cryogenic performance of the HSPD, and increasing modulation depth.
